Cosmological Perturbations in the Early Universe

One essence in capturing the history of primordial fluctuations that arise during inflation and eventually lead to formation of large scale structures in the universe, relies on quantizing general relativity coupled to a scalar field. This is a system that respects diffeomorphism invariance, the freedom of choosing the coordinate system to work with without changing the physics. Hence the way to handle its quantization requires an understanding of how to quantize diffeomorphisms.Deciding on suitable coordinate choices and making sure that this gauge fixing, which is unavoidable in any calculation, does not effect the end result, is tricky. In this thesis we make full use of the effects of diffeomorphism invariance of the theory on the primordial fluctuations to pursue two different approaches that focus on treating perturbations after gauge fixing. On one hand we work towards developing our understanding of how to handle quantization in terms of Dirac quantization and Becchi, Rouet, Stora, Tyutin (BRST) quantization. On another, we focus on how to generalize the allowed interactions and understand the scales they bring in the era of preheating that follows inflation, with effective field theory (EFT) methods on cosmological backgrounds.

==> Makefile <==
TEXFILES= conclusions.tex \
detectors.tex \
eobpn_1-5pnmetric_effectualness.tex \
imr_IMRI.tex \
inspiral_IMRI.tex \
introduction.tex \
ninja2.tex \
nrhyb_tmpltbank.tex \
theory.tex \
thesis.tex 


PNGFILES=figures/detchar/966222827_940673828_H0_PEM-ISCT1_ACCX_1_00_spectrogram_whitened.png \
figures/detchar/966222827_940673828_H1_LSC-DARM_ERR_1_00_spectrogram_whitened.png \
figures/detchar/968654557_978027343_L1_LSC-DARM_ERR_1_00_spectrogram_whitened.png \
figures/detchar/968654557_997314453_H1_LSC-DARM_ERR_1_00_spectrogram_whitened.png \
figures/detchar/frontendtest_h1_log_2.png \
figures/detchar/frontendtest_l1_log_2.png \
figures/detchar/frontendtest_v1_log_2.png \
figures/detchar/GAUSSIAN_0_UNCLUSTERED_chisq.png \
figures/detchar/H1_0_UNCLUSTERED_chisq.png \
figures/detchar/H1_0_UNCLUSTERED_rate_vs_time.png \
figures/detchar/H1_0_UNCLUSTERED_snr_vs_time.png \
figures/detchar/H1_1_UNCLUSTERED_chisq.png \
figures/detchar/H1_1_UNCLUSTERED_glitchgram.png \
figures/detchar/H1_1_UNCLUSTERED_snr_hist.png \
figures/detchar/H1_4_UNCLUSTERED_chisq.png \
figures/detchar/H1_4_UNCLUSTERED_snr_hist.png \
figures/detchar/hybrid_bank.png \
figures/detchar/LM_H1_16SEC_3_hist.png \
figures/detchar/LM_H1_30MILLISEC_3_hist.png \
figures/detchar/LM_L1_16SEC_3_hist.png \
figures/detchar/LM_L1_30MILLISEC_3_hist.png \
figures/detchar/loudest.png \
figures/detchar/MM_H1_16SEC_3_hist.png \
figures/detchar/MM_H1_30MILLISEC_3_hist.png \
figures/detchar/MM_L1_16SEC_3_hist.png \
figures/detchar/MM_L1_30MILLISEC_3_hist.png \
figures/detchar/vetousage.png

BIBFILES=references.bib

STYFILES=bibunits.sty syrthesis.sty

BSTFILES=

BBLFILES=

default: clean thesis.pdf

thesis.pdf: $(TEXFILES) $(BIBFILES) $(STYFILES) $(BSTFILES)
	pdflatex thesis && bibtex thesis && bibtex thesis && pdflatex thesis && pdflatex thesis

gr-qc: thesis.tgz

thesis.tgz: thesis.pdf
	tar -zcvf grqc.tgz $(TEXFILES) $(PNGFILES) $(BBLFILES) $(STYFILES)

clean:
	rm -f thesis.pdf *.aux *.bbl *.blg *.log *.lot *.toc *.lof *.bak *.tgz *.out


==> list_pubs.tex <==
\vspace*{2em}
This dissertation includes the following three peer-reviewed and published articles:
\begin{enumerate}
	\item{``Nonthermal WIMPs and primordial black holes'', Julian Georg, Gizem Şengör, Scott Watson, Phys.Rev. D93 (2016) no.12, 123523, arXiv:1603.00023 [hep-ph]}
	
\item{``BRST Quantization of Cosmological Perturbations'', Cristian Armendariz-Picon, Gizem Şengör, JCAP 1611 (2016) no.11, 016,  arXiv:1606.03823 [hep-th] }

\item{``Toward an Effective Field Theory Approach to Reheating'', Ogan Özsoy, John T. Giblin, Eva Nesbit, Gizem Şengör, Scott Watson,	Phys.Rev. D96 (2017) no.12, 123524,
	arXiv:1701.01455 [hep-th]}
\end{enumerate}


